GRIN: Zero-Shot Metric Depth with Pixel-Level Diffusion

3D reconstruction from a single image is a long-standing problem in computer vision. Learning-based methods address its inherent scale ambiguity by leveraging increasingly large labeled and unlabeled datasets, to produce geometric priors capable of generating accurate predictions across domains. As a result, state of the art approaches show impressive performance in zero-shot relative and metric depth estimation. Recently, diffusion models have exhibited remarkable scalability and generalizable properties in their learned representations. However, because these models repurpose tools originally designed for image generation, they can only operate on dense ground-truth, which is not available for most depth labels, especially in real-world settings. In this paper we present GRIN, an efficient diffusion model designed to ingest sparse unstructured training data. We use image features with 3D geometric positional encodings to condition the diffusion process both globally and locally, generating depth predictions at a pixel-level. With comprehensive experiments across eight indoor and outdoor datasets, we show that GRIN establishes a new state of the art in zero-shot metric monocular depth estimation even when trained from scratch.

==> figures/embeddings.tex <==
\begin{figure}[t!]
\begin{center}
\subfloat[Global Image Embeddings.]{
\label{fig:global_embeddings}
\includegraphics[width=0.35\textwidth]{assets/images/image_embeddings_global.png}
}
\subfloat[Local Image Embeddings.]{
\label{fig:local_embeddings}
\includegraphics[width=0.20\textwidth]{assets/images/image_embeddings_local.png}
}
\subfloat[Geometric Embeddings.]{
\label{fig:geometric_embeddings}
\includegraphics[width=0.35\textwidth]{assets/images/geometric_embeddings.png}
}
\caption{\textbf{Input-level embeddings} used to condition the GRIN diffusion process. (a) Global image embeddings are generated using a convolutional encoder $\mathcal{F}_{\theta}$ to produce multi-scale features, that are upsampled and concatenated to generate a $\frac{H}{4} \times \frac{W}{4} \times 960$ feature map $\textbf{F}_i^g = \mathcal{F}_{\theta}^g(I_i)$. (b) Local image embeddings are generated at a patch-level, using a single convolutional layer with a $9 \times 9$ kernel to generate $128$-dimensional features $\textbf{f}_{ijk}^l$ for each pixel $(u,v)_{jk}$ from image $I_i$. (c) Geometric embeddings are generated by Fourier-encoding the camera center $\textbf{t}_i$ (shared across all pixels from image $I_i$) as well as per-pixel viewing rays $\textbf{r}_{ijk}$, based on camera intrinsics $\textbf{K}_i$ and extrinsics $\textbf{T}_i$.
}
\vspace{-5mm}
\label{fig:embeddings}
\end{center}
\end{figure}
